Concept for an Electron Ion Collider (EIC) detector built around the BaBar solenoid

The PHENIX collaboration presents here a concept for a detector at a future Electron Ion Collider (EIC). The EIC detector proposed here, referred to as ePHENIX, will have excellent performance for a broad range of exciting EIC physics measurements, providing powerful investigations not currently available that will dramatically advance our understanding of how quantum chromodynamics binds the proton and forms nuclear matter.

==> detector_performance.tex <==
\chapter{Performance of the sPHENIX Detector}
\label{chap:detector_performance}




